Kinematic analysis of the super-extended HI disk of the nearby spiral galaxy M83

We present new HI observations of the nearby massive spiral galaxy M83, taken with the VLA at $21^{\prime\prime}$ angular resolution ($\approx500$ pc) of an extended ($\sim$1.5 deg$^2$) 10-point mosaic combined with GBT single dish data. We study the super-extended HI disk of M83 (${\sim}$50 kpc in radius), in particular disc kinematics, rotation and the turbulent nature of the atomic interstellar medium. We define distinct regions in the outer disk ($r_{\rm gal}>$central optical disk), including ring, southern area, and southern and northern arm. We examine HI gas surface density, velocity dispersion and non-circular motions in the outskirts, which we compare to the inner optical disk. We find an increase of velocity dispersion ($\sigma_v$) towards the pronounced HI ring, indicative of more turbulent HI gas. Additionally, we report over a large galactocentric radius range (until $r_{\rm gal}{\sim}$50 kpc) that $\sigma_v$ is slightly larger than thermal (i.e. $>8$km s$^{-1}$ ). We find that a higher star formation rate (as traced by FUV emission) is not always necessarily associated with a higher HI velocity dispersion, suggesting that radial transport could be a dominant driver for the enhanced velocity dispersion. We further find a possible branch that connects the extended HI disk to the dwarf irregular galaxy UGCA365, that deviates from the general direction of the northern arm. Lastly, we compare mass flow rate profiles (based on 2D and 3D tilted ring models) and find evidence for outflowing gas at r$_{\rm gal}$ $\sim$2 kpc, inflowing gas at r$_{\rm gal}$ $\sim$5.5 kpc and outflowing gas at r$_{\rm gal}$ $\sim$14 kpc. We caution that mass flow rates are highly sensitive to the assumed kinematic disk parameters, in particular, to the inclination.

==> Figures/01caption/figure-model_parameters.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/plots/Heald16_incl46.png}
    \caption{\textbf{The model outputs from \cite{Heald2016}.} We take them to construct the synthetic velocity map show in \autoref{fig:mom1}  }
    \label{fig:model_parameters}
\end{figure*}

==> Figures/01caption/figure-vlos.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Figures/plots/asymmetry_vlos.pdf}
    \caption{The observed velocities, \vlosobs\ in grey and modeled velocities \vlosmdl\ in purple. We marked here a peak of approaching \vlosobs\ (blue shaded area) and a lack of approaching \vlosobs\ (beyond galactocentric radius of 47~kpc) values. The symmetry breaks at ${\sim}$22~kpc, see \autoref{appendix:add_figures}}
    \label{fig:vlos_vsyn}
\end{figure}

==> Table/table-observations_referee.tex <==
\begin{table*}[]
\centering
\caption{Summary of our VLA $\hi$ observation across \gal. }
\label{tab:observation}
\begin{tabular}{lccc|cc|cc|ccc}
\hline \hline
\multicolumn{1}{c}{}  &
  $\nu_{\rm rest}$ &
  \begin{tabular}[c]{@{}c@{}}project\\ codes\end{tabular} &
  \begin{tabular}[c]{@{}c@{}} sessions\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}gain/phase\\ calibrator\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}bandpass/flux\\ calibrator\end{tabular} &
  Configuration &
  \begin{tabular}[c]{@{}c@{}}obs. time \\ per Config.\end{tabular} &
  \begin{tabular}[c]{@{}c@{}} total \\ obs. \\ time\end{tabular} & 
  \begin{tabular}[c]{@{}c@{}}total \\ on\\ source\end{tabular}\\
\multicolumn{1}{c}{\multirow{-2}{*}{}} & [MHz] & & & &  &  & [min] & [min] & [min]   \\
& (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9)   \\ \hline
\hi\   & 1420.4058 & 13B-194 & 17 &J1311-2216     &  1331+305=3C286         & BnA   & 378  &  2406  & 1444  \\
&  & and & & and &  & CnB   & 516  & &       \\
&  & 14B-192 & 5 & J1316-3338&  & DnC   & 1512 & &      \\
\hline 
\end{tabular}
 \begin{minipage}{1.0\columnwidth}
        \vspace{1mm}
        {\bf Notes.} Column (1): Observational frequency. (2--3): The project codes and the corresponding number of observation sessions (PI: F. Bigiel). (4): The sources we used to calibrate the gain (amplitude and phase). (5): The source we used to perform the bandpass (flux and delay) calibration. (6--9): We quote here the outputs using \texttt{analysisUtils} after we have flagged our data: (6--7): Time of the observation per configuration. (8): Total observation time. (9): Total on source time. 
    \end{minipage}
\end{table*}

